Improving Protein Optimization with Smoothed Fitness Landscapes

The ability to engineer novel proteins with higher fitness for a desired property would be revolutionary for biotechnology and medicine. Modeling the combinatorially large space of sequences is infeasible; prior methods often constrain optimization to a small mutational radius, but this drastically limits the design space. Instead of heuristics, we propose smoothing the fitness landscape to facilitate protein optimization. First, we formulate protein fitness as a graph signal then use Tikunov regularization to smooth the fitness landscape. We find optimizing in this smoothed landscape leads to improved performance across multiple methods in the GFP and AAV benchmarks. Second, we achieve state-of-the-art results utilizing discrete energy-based models and MCMC in the smoothed landscape. Our method, called Gibbs sampling with Graph-based Smoothing (GGS), demonstrates a unique ability to achieve 2.5 fold fitness improvement (with in-silico evaluation) over its training set. GGS demonstrates potential to optimize proteins in the limited data regime. Code: https://github.com/kirjner/GGS

==> experiments/ablation.tex <==
\TODO{Andrew, update}
We perform ablations on the two stages of \method on the hard difficulty task.
In the first ablation, we remove \smoothing and start sampling after initial predictor training. 
The second ablation runs \extrapolation for fewer that 15 iterations (1, 5, and 10).

Our results are shown in \Cref{table:ablations}.
We see GS is crucial for \method on the hard difficulty level.
When \extrapolation is run for 1 or 5 iterations there is also a large decrease in performance. Running \extrapolation for    10 iterations achieves equivalent fitness, but slightly worse diversity and novelty. 
We conclude each component of \method contributes to its performance.
\begin{table*}[!ht]
  \vspace{-11pt}
  \caption{Ablation results (our oracle).}
  \label{table:ablations}
  \centering
  \begin{tabular}{ll|ccccc}
    \toprule
    Difficulty & Metric & \textbf{\method} &  without GS &  IE10 & IE5 & IE1  \\
    \cmidrule(lr){1-7}
    \multirow{3}{*}{Hard} & Fitness & 
    \textbf{0.81 (0.0)}  & -0.03 (0.0) & \textbf{0.81 (0.0)} & 0.40 (0.0) & 0.07 (0.0)\\
    & Diversity & 2.6 (0.0)  & 22.7 (1.6)  & 2.5 (0.0) & 5.7 (0.0) & 13.5 (0.0) \\
    & Novelty & 7.0 (0.0)  & 13.4 (0.5) & 6.7 (0.4) & 5.0 (0.0) & 1.0 (0.0)   \\

    \bottomrule
  \end{tabular}
\end{table*}


==> method/iterative_extrapolation.tex <==

The 1st order Taylor approximation of \cref{eq:big_proposal} deteriorates the more we mutate from the parent sequence.
Inspired by directed evolution \citep{arnold1998design}, we propose to alleviate this by performing multiple rounds of sampling where successive rounds use sequences from the previous round.
Each round re-centers the Taylor approximation and applies another round of \sampling.
We first train a predictor $\model$ using GS (\Cref{sec:smoothing}).
Prior to sampling, we observe the number of sequences may be large and redundant.
To reduce the number of sequences, we perform hierarchical clustering \citep{mullner2011modern} and take the sequence of each cluster with the highest fitness using $\model$. Let $\numclusters$ be the number of clusters.
\begin{equation}
    \texttt{Reduce}(\
     \{\seqset^c\}_{c=1}^\numclusters; \theta) = \bigcup_{c = 1}^\numclusters \{\argmax_{\seq \in \seqset^c} \model(\seq)\} \ \text{ where } \
     \{\seqset^c\}_{c=1}^\numclusters = \texttt{Cluster}(\seqset; \numclusters).
\end{equation}
Each round $r$ reduces the sequences from the previous round and performs \sampling sampling.
% \begin{equation}
    % \label{eq:ie_rounds}
\begin{equation}
    % \text{For round $r \in \{0,\dots, \numrounds\}$: } 
    \seqset_{r+1}'= \bigcup_{\seq \in \tilde{\seqset}_r}\texttt{\sampling}(\seq; \theta),\quad \tilde{\seqset}_r = \texttt{Reduce}(\{\seqset^c_r\}_{c=1}^\numclusters; \theta), \quad \{\seqset^c_r\}_{c=1}^\numclusters = \texttt{Cluster}(\seqset_r'; \numclusters).
\end{equation}
One cycle of clustering, reducing, and sampling is a round of extrapolation,
\begin{equation}
    \seqset_{r+1}' = \texttt{Extrapolate}(\seqset_{r}'; \theta, \mathcal{C}) \label{eq:ie_rounds}
\end{equation}
% \end{equation}
where the initial round $r=0$ starts with $\seqset_0' = \seqset_0$.
% \begin{align}
%     &\text{\textbf{First round}: $r=0$} &\seqset_{1}'= \bigcup_{\seq \in \tilde{\seqset}_0} \texttt{\sampling}(\seq; \theta),\quad &\tilde{\seqset}_0 = \texttt{Reduce}(\seqset_0; \theta, \numclusters) \label{eq:ie_initial}\\
%     &\text{\textbf{For round} $r \in \{1,\dots, \numrounds\}$: } &\seqset_{r+1}'= \bigcup_{\seq \in \tilde{\seqset}_r}\texttt{\sampling}(\seq; \theta),\quad &\tilde{\seqset}_r = \texttt{Reduce}(\seqset_r'; \theta, \numclusters), \label{eq:ie_rounds}
% \end{align}
After $\numrounds$ rounds, we select our candidate sequences by taking the Top-$\numcandidates$ sequences based on ranking with $\model$.
We call this procedure Iterative Extrapolation (IE).
While IE is related to previous directed evolution methods \cite{sinai2020adalead}, it differs in that it encourages diversity by mutating the best sequence of each cluster.
The full candidate generation, Gibbs with Graph-based Smoothing (\method), with IE is presented in \Cref{alg:generation}.




==> method/protein_fitness_refinement.tex <==
\label{protein_fitness_refinement}
PFR consists of three key steps:
\\\\
 \textbf{Regression}. In the regression step, we train a base model, which we denote $f_{base}$ on the sequences in $\mathcal{X}$ in a supervised fashion to predict the corresponding sequences in $\mathcal{Y}$. The base model in PFR consists of an input convolutional layer that takes in a one-hot encoded sequence $x$, which corresponds to the amino-acid seqeunce $x \in \mathcal{X}$ followed by max-pooling, followed by a  dense layer to a single output node that outputs  $f_{base}(x)$, the base model's prediction of the corresponding fitness $y$. We also use a negative data augmentation strategy during the training process to reduce false positives. The goal is to use this base model to score new candidate sequences, which are produced via the generation scheme below, and leverage these scores to identify improvements over the original sequences in $\mathcal{X}$. \\\\ 
 \textbf{Generation}. To generate new sequences, we utilize a modified version of the Gibbs With Gradient (GWG) approach introduced in \cite{grathwohl2021oops}. For a given one-hot encoded sequence $x$ that is represented by an $L \times V$ matrix, where the $L$ is the length of $x$ and $V$ is the size of the amino acid vocabulary (usually 20), we generate candidate sequences as follows: We consider the binary entries in its one-hot encoding matrix, of size $L \times V$ as continuous variables, so that we may compute the gradients of these entries with respect to our base model in order to sample candidates that are likely to be improvements.  We may then compute for $i \in \{1,...,L\}$, $j \in \{1,...,V\}$ the matrix $\delta \in \mathbb{R}^{L\times V}$
\[\delta_{ij} = \nabla_xf_{base}(x)_{ij} -  x_i^T\nabla f_{base}(x)_ix \]
Framing this problem in the context of (log) likelihood-maximization, where $f_{base}(\cdot)$ represents the unnormalized (log) probability over all possible sequences of length $L$, then these $\delta_ij$ represent a first-order approximation of the(log) likelihood ratios of changing the amino acid at dimension $i$ from its current state to the $j$th amino acid in the vocabulary. We then use the $\delta_{ij}$ to generate potential candidates for each sequence $x$, which we consider to be length-$L$ sequences that are at most $m$ mutations away from this $x$, where $m \in \{1,...,M\}$, where $M$ is the maximal number of mutations we consider. For a given pair $(x, m)$, we employ a bi-level sampling scheme to generate new candidates to be scored by our base model. At the first level, sample the positions we wish to alter from the set $\{1,...,L\}$. We do this by first considering the row-wise maxima, $\delta_{i} = \max_j \delta_{ij}$. These represent the approximate maximal fitness improvement that comes from altering the amino acid at position $i$. We then sample a set of  $m$ positions (potentially with replacement) from the following categorical distribution 
\[\mathcal{I} = \{i_1,...,i_m\} \stackrel{iid}{\sim}\text{Cat}\left(\text{Softmax}\left(\frac{\delta_1,...,\delta_L}{\tau_{pos}}\right)\right)\]
Where $\tau_{pos}$ is a temperature parameter that modulates positional exploration. Because we sample with replacement, it is possible that $|\mathcal{I}| < m$, but we consider for the moment the case where $|\mathcal{I}| = m$. At the second level, we take these $m$ positions, and sample new candidates $\{\tilde{x}_1,...\tilde{x}_m\}$
\[\tilde{x}_l \sim \text{Cat}\left(\text{Softmax}\left(\frac{\delta_{l1},...\delta_{lV}}{\tau_{AA}}\right)\right)\]
for each $l \in \mathcal{I}$. Here, $\tau_{AA}$ is a is a temperature parameter that modulates AA exploration at a given position.\textcolor{red}{again, notation could be cleaned up}. For each of these new candidates $\tilde{x}$, we score the fitness  using the base model and add it to an accepted set $\mathcal{A}$ if
\[f_{base}(\tilde{x}) - f_{base}(x) > \epsilon\]
Where $\epsilon > 0$ is an \textit{edit tolerance} that reduces noise from the base model scores, which are only an approximation of fitness. Finally, each accepted $\tilde{x}$ is also added to our original set $\mathcal{X}$, as this allows for increased exploration of the fitness landscape. This process is repeated for $T$ iterations over all $m \in \{1,...,M\}$ and all $x$ in the set $\mathcal{X}$, the latter of which may grow after each iteration. The generation step is summarized in Algorithm 1.
\\\\
 \textbf{Selection}.
In the final step, we use our $f_{base}$ to score each of the sequences in $\mathcal{A}$, and select the Top-$K$ scoring sequences as our final candidates. \\\\
Following regression, generation, and selection, we use the appropriate oracle to evaluate the final candidates on the criteria described above. 
